PromptIntern: Saving Inference Costs by Internalizing Recurrent Prompt during Large Language Model Fine-tuning

Recent advances in fine-tuning large language models (LLMs) have greatly enhanced their usage in domain-specific tasks. Despite the success, fine-tuning continues to rely on repeated and lengthy prompts, which escalate computational expenses, require more resources, and lead to slower inference. In this paper, we present a novel approach, PromptIntern, which internalizes prompt knowledge during model fine-tuning to achieve efficient inference and save costs. Instead of compressing the prompts for a vanilla model, PromptIntern aims to embed the recurrent prompt directly into the model parameters. We design a fine-tuning pipeline that includes instruction template compression, few-shot example absorption, and a progressive internalization strategy, effectively diminishing the need for intricate prompts during inference. Comprehensive experiments on challenging NL2Code tasks demonstrate that our method reduces input tokens by more than 90%, accelerates inference by 4.2 times, and reduces monetary inference costs by 88.3%.

==> source/tables/mbpp_cost_template.tex <==
% \begin{table*}[!t]
%   \centering
%   \label{tab:mbpp_cost_template}
%   \caption{Results of Various Models Using PromptIntern on MBPP}
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{4}{c}{\textbf{Inference Time (s/instance)}} & \multicolumn{4}{c}{\textbf{Token Number (per instance)}} \\ 
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     & \textbf{x1.0} & \textbf{x0.6} & \textbf{x0.3} & \textbf{x1.0-0.6-0.3} & \textbf{x1.0} & \textbf{x0.6} & \textbf{x0.3} & \textbf{x1.0-0.6-0.3} \\
%     \midrule
%     GPT-4  & 0.67 & 0.67 & 0.63 & 0.61 & 272 & 179 & 89 & 89 \\
%     GPT-3.5 & 0.41 & 0.37 & 0.36 & 0.36 & 272 & 179 & 89 & 89 \\
%     Llama2-7B  & 0.51 & 0.46 & 0.27 & 0.27 & 311 & 191 & 95 & 95 \\
%     Llama2-13B  & 1.48 & 1.32 & 0.86 & 0.82 & 320 & 196 & 104 & 104 \\
%     Mixtual-8x7B  & 1.72 & 1.43 & 0.85 & 0.85 & 320 & 196 & 104 & 104 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table*}


















==> source/tables/nl2b_res.tex <==
\begin{table*}[!t]
  \centering
  \caption{Comparison with direct fine-tuning baselines on NL2Bash datasets.}
  \label{tab:nl2bash_res}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{Template \textit{with} 10-shots} & \multicolumn{2}{c}{Template x0.6 \textit{with} 5-shots} & \multicolumn{2}{c}{Template Only}  & \multicolumn{2}{c}{No Template}& \multicolumn{2}{c}{\textbf{\our}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
    & BLEU & Tokens & BLEU & Tokens  & BLEU & Tokens  & BLEU & Tokens & \textbf{BLEU} & \textbf{Tokens} \\
    \midrule
        GPT-4 & 86.7 & 1063 & 81.3 & 810 & 78.6 & 484 & 71.2 & 52 & \textbf{82.5} & \textbf{52} \\ 
        GPT-3.5 & 74.2 & 1063 & 67.5 & 810 & 65.1 & 484 & 61.2 & 52 & \textbf{67.7} & \textbf{52} \\ 
        Mixtral-8x7B & 63.8 & 1320 & 58.3 & 1053 & 54.9 & 603 & 47.6 & 68 & \textbf{57.2} & \textbf{68} \\ 
        Llama2-13B & 47.1 & 1244 & 43.9 & 988 & 41.6 & 574 & 35.1 & 64 & \textbf{43.5} & \textbf{64} \\ 
        Llama2-7B & 35.8 & 1244 & 32.7 & 988 & 31.4 & 574 & 22.1 & 64 & \textbf{31.6} & \textbf{64} \\ 
    \bottomrule
    \end{tabular}
  }
\end{table*}





    

==> source/tables/nl2f_res.tex <==
\begin{table*}[!t]
  \centering
  \caption{Comparison with direct fine-tuning baselines on NL2F datasets.}
  \label{tab:nl2f_res}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{Template \textit{with} 10-shots} & \multicolumn{2}{c}{Template x0.6 \textit{with} 5-shots} & \multicolumn{2}{c}{Template Only}  & \multicolumn{2}{c}{No Template}& \multicolumn{2}{c}{\textbf{\our}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
    & E.M. & Tokens & E.M. & Tokens  & E.M. & Tokens  & E.M. & Tokens & \textbf{E.M.} & \textbf{Tokens} \\
    \midrule
        GPT-4 & 94.8 & 3540 & 92.1 & 1838 & 89.7 & 680 & 82.5 & 286 & \textbf{91.6} & \textbf{286} \\ 
        GPT-3.5 & 85.5 & 3540 & 78.1 & 1838 & 76.2 & 680 & 70.4 & 286 & \textbf{78.4} & \textbf{286} \\ 
        Mixtral-8x7B & 69.3 & 4204 & 66.3 & 2191 & 63.8 & 814 & 54.2 & 339 & \textbf{65.2} & \textbf{339} \\ 
        Llama2-13B & 59.2 & 4202 & 54.9 & 2183 & 54.1 & 812 & 32.9 & 339 & \textbf{55.3} & \textbf{339} \\ 
        Llama2-7B & 45.4 & 4202 & 40.7 & 2183 & 38.5 & 812 & 21.8 & 339 & \textbf{40.8} & \textbf{339} \\ 
    \bottomrule
    \end{tabular}
  }
\end{table*}


    
